Stein Block Thresholding For Image Denoising

In this paper, we investigate the minimax properties of Stein block thresholding in any dimension $d$ with a particular emphasis on $d=2$. Towards this goal, we consider a frame coefficient space over which minimaxity is proved. The choice of this space is inspired by the characterization provided in \cite{BorupNielsen} of family of smoothness spaces on $\mathbb{R}^d$, a subclass of so-called decomposition spaces \cite{Feichtinger}. These smoothness spaces cover the classical case of Besov spaces, as well as smoothness spaces corresponding to curvelet-type constructions. Our main theoretical result investigates the minimax rates over these decomposition spaces, and shows that our block estimator can achieve the optimal minimax rate, or is at least nearly-minimax (up to a $\log$ factor) in the least favorable situation. Another contribution is that the minimax rates given here are stated for a general noise sequence model in the transform coefficient domain beyond the usual i.i.d. Gaussian case. The choice of the threshold parameter is theoretically discussed and its optimal value is stated for some noise models such as the (non-necessarily i.i.d.) Gaussian case. We provide a simple, fast and a practical procedure. We also report a comprehensive simulation study to support our theoretical findings. The practical performance of our Stein block denoising compares very favorably to the BLS-GSM state-of-the art denoising algorithm on a large set of test images. A toolbox is made available for download on the Internet to reproduce the results discussed in this paper.

==> images/CURV_barbara512x512.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{BARBARA512X512 with CURV}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&36.68&37.17&35.05&34.36\\\hline
\textbf{  3}&34.15&35.78&37.57&35.48&34.46\\\hline
\textbf{  4}&34.15&35.09&37.46&35.89&34.56\\\hline
\textbf{4.5}&34.15&34.80&37.33&36.08&34.62\\\hline
\textbf{  5}&34.15&34.54&37.17&36.27&34.67\\\hline
\textbf{  6}&34.15&34.08&36.83&36.60&34.77\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&33.01&32.78&29.40&28.43\\\hline
\textbf{  3}&28.13&32.15&33.64&30.05&28.58\\\hline
\textbf{  4}&28.14&31.47&33.68&30.70&28.73\\\hline
\textbf{4.5}&28.14&31.19&33.56&31.01&28.81\\\hline
\textbf{  5}&28.14&30.93&33.42&31.32&28.89\\\hline
\textbf{  6}&28.14&30.48&33.09&31.91&29.04\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&30.93&30.15&26.05&24.95\\\hline
\textbf{  3}&24.61&30.07&31.37&26.81&25.13\\\hline
\textbf{  4}&24.61&29.39&31.53&27.59&25.30\\\hline
\textbf{4.5}&24.61&29.11&31.44&27.98&25.39\\\hline
\textbf{  5}&24.61&28.86&31.30&28.36&25.48\\\hline
\textbf{  6}&24.61&28.42&30.98&29.11&25.66\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&29.43&28.21&23.65&22.47\\\hline
\textbf{  3}&22.11&28.61&29.72&24.48&22.66\\\hline
\textbf{  4}&22.11&27.95&29.99&25.34&22.85\\\hline
\textbf{4.5}&22.11&27.67&29.92&25.77&22.95\\\hline
\textbf{  5}&22.11&27.43&29.79&26.21&23.05\\\hline
\textbf{  6}&22.11&27.01&29.48&27.07&23.24\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&28.30&26.70&21.78&20.56\\\hline
\textbf{  3}&20.17&27.49&28.44&22.66&20.75\\\hline
\textbf{  4}&20.18&26.85&28.82&23.58&20.96\\\hline
\textbf{4.5}&20.18&26.58&28.77&24.05&21.06\\\hline
\textbf{  5}&20.18&26.34&28.65&24.53&21.16\\\hline
\textbf{  6}&20.18&25.93&28.35&25.48&21.37\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&27.37&25.43&20.25&18.99\\\hline
\textbf{  3}&18.59&26.59&27.38&21.16&19.19\\\hline
\textbf{  4}&18.59&25.96&27.86&22.12&19.40\\\hline
\textbf{4.5}&18.59&25.71&27.82&22.62&19.50\\\hline
\textbf{  5}&18.59&25.48&27.71&23.13&19.61\\\hline
\textbf{  6}&18.60&25.09&27.42&24.15&19.83\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&24.80&21.71&15.91&14.57\\\hline
\textbf{  3}&14.15&24.16&24.28&16.90&14.79\\\hline
\textbf{  4}&14.15&23.64&25.13&17.96&15.02\\\hline
\textbf{4.5}&14.16&23.43&25.18&18.52&15.13\\\hline
\textbf{  5}&14.16&23.25&25.13&19.10&15.24\\\hline
\textbf{  6}&14.16&22.97&24.90&20.30&15.48\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&21.50&16.37&9.98&8.58\\\hline
\textbf{  3}&8.14&21.31&19.77&11.03&8.81\\\hline
\textbf{  4}&8.14&21.10&21.31&12.18&9.05\\\hline
\textbf{4.5}&8.14&21.03&21.58&12.80&9.17\\\hline
\textbf{  5}&8.14&20.97&21.68&13.45&9.29\\\hline
\textbf{  6}&8.14&20.90&21.65&14.82&9.54\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/CURV_boat.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{BOAT with CURV}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&35.73&36.65&34.93&34.34\\\hline
\textbf{  3}&34.15&34.80&36.88&35.30&34.43\\\hline
\textbf{  4}&34.15&34.12&36.65&35.65&34.53\\\hline
\textbf{4.5}&34.15&33.84&36.46&35.81&34.57\\\hline
\textbf{  5}&34.15&33.60&36.26&35.96&34.62\\\hline
\textbf{  6}&34.15&33.17&35.86&36.23&34.71\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.14&32.32&32.42&29.36&28.43\\\hline
\textbf{  3}&28.14&31.47&33.09&29.97&28.58\\\hline
\textbf{  4}&28.14&30.84&33.01&30.58&28.73\\\hline
\textbf{4.5}&28.14&30.57&32.87&30.87&28.81\\\hline
\textbf{  5}&28.14&30.34&32.70&31.16&28.88\\\hline
\textbf{  6}&28.14&29.94&32.36&31.69&29.03\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&30.44&29.92&26.03&24.96\\\hline
\textbf{  3}&24.62&29.64&30.96&26.78&25.13\\\hline
\textbf{  4}&24.62&29.04&31.03&27.53&25.31\\\hline
\textbf{4.5}&24.62&28.79&30.91&27.91&25.40\\\hline
\textbf{  5}&24.62&28.57&30.76&28.28&25.49\\\hline
\textbf{  6}&24.62&28.19&30.43&28.99&25.67\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&29.15&28.08&23.64&22.48\\\hline
\textbf{  3}&22.11&28.39&29.45&24.47&22.67\\\hline
\textbf{  4}&22.11&27.82&29.65&25.32&22.86\\\hline
\textbf{4.5}&22.11&27.59&29.55&25.75&22.96\\\hline
\textbf{  5}&22.11&27.38&29.42&26.18&23.06\\\hline
\textbf{  6}&22.12&27.03&29.10&27.03&23.26\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.18&28.17&26.62&21.79&20.57\\\hline
\textbf{  3}&20.18&27.45&28.27&22.67&20.77\\\hline
\textbf{  4}&20.18&26.90&28.58&23.58&20.97\\\hline
\textbf{4.5}&20.18&26.69&28.52&24.05&21.07\\\hline
\textbf{  5}&20.18&26.49&28.39&24.53&21.18\\\hline
\textbf{  6}&20.18&26.17&28.10&25.48&21.39\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&27.37&25.39&20.26&18.99\\\hline
\textbf{  3}&18.60&26.70&27.27&21.17&19.20\\\hline
\textbf{  4}&18.60&26.19&27.70&22.14&19.41\\\hline
\textbf{4.5}&18.60&25.99&27.66&22.64&19.52\\\hline
\textbf{  5}&18.60&25.81&27.56&23.15&19.63\\\hline
\textbf{  6}&18.60&25.52&27.28&24.17&19.85\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&25.18&21.76&15.93&14.58\\\hline
\textbf{  3}&14.16&24.73&24.36&16.92&14.80\\\hline
\textbf{  4}&14.16&24.35&25.24&18.00&15.03\\\hline
\textbf{4.5}&14.16&24.21&25.32&18.56&15.15\\\hline
\textbf{  5}&14.16&24.09&25.29&19.15&15.26\\\hline
\textbf{  6}&14.16&23.89&25.11&20.36&15.50\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&22.12&16.45&9.99&8.58\\\hline
\textbf{  3}&8.13&22.10&19.95&11.05&8.81\\\hline
\textbf{  4}&8.14&21.96&21.64&12.21&9.05\\\hline
\textbf{4.5}&8.14&21.90&21.98&12.83&9.17\\\hline
\textbf{  5}&8.14&21.86&22.14&13.49&9.29\\\hline
\textbf{  6}&8.14&21.79&22.20&14.87&9.54\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/CURV_fingerprint.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{FINGERPRINT with CURV}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&34.90&35.99&34.75&34.30\\\hline
\textbf{  3}&34.15&33.89&36.13&35.03&34.38\\\hline
\textbf{  4}&34.15&33.12&35.91&35.29&34.45\\\hline
\textbf{4.5}&34.15&32.80&35.73&35.41&34.49\\\hline
\textbf{  5}&34.15&32.51&35.53&35.52&34.53\\\hline
\textbf{  6}&34.15&32.01&35.13&35.72&34.60\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&30.87&31.54&29.18&28.39\\\hline
\textbf{  3}&28.13&29.87&31.98&29.69&28.52\\\hline
\textbf{  4}&28.13&29.09&31.85&30.19&28.65\\\hline
\textbf{4.5}&28.13&28.77&31.69&30.43&28.72\\\hline
\textbf{  5}&28.13&28.48&31.52&30.65&28.79\\\hline
\textbf{  6}&28.14&27.98&31.16&31.07&28.92\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&28.61&28.96&25.87&24.92\\\hline
\textbf{  3}&24.61&27.64&29.65&26.52&25.08\\\hline
\textbf{  4}&24.61&26.92&29.58&27.16&25.24\\\hline
\textbf{4.5}&24.61&26.64&29.42&27.48&25.32\\\hline
\textbf{  5}&24.61&26.38&29.24&27.78&25.40\\\hline
\textbf{  6}&24.61&25.96&28.85&28.36&25.56\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.12&27.12&27.14&23.52&22.46\\\hline
\textbf{  3}&22.12&26.23&28.04&24.25&22.64\\\hline
\textbf{  4}&22.12&25.59&28.01&24.99&22.81\\\hline
\textbf{4.5}&22.12&25.33&27.86&25.36&22.90\\\hline
\textbf{  5}&22.12&25.11&27.68&25.72&22.99\\\hline
\textbf{  6}&22.12&24.74&27.29&26.42&23.17\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.18&26.04&25.70&21.67&20.55\\\hline
\textbf{  3}&20.18&25.22&26.80&22.47&20.73\\\hline
\textbf{  4}&20.18&24.64&26.84&23.28&20.92\\\hline
\textbf{4.5}&20.19&24.42&26.71&23.69&21.02\\\hline
\textbf{  5}&20.19&24.22&26.54&24.09&21.11\\\hline
\textbf{  6}&20.19&23.89&26.18&24.88&21.31\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&25.22&24.49&20.14&18.97\\\hline
\textbf{  3}&18.59&24.47&25.79&20.98&19.16\\\hline
\textbf{  4}&18.59&23.94&25.92&21.85&19.36\\\hline
\textbf{4.5}&18.59&23.73&25.81&22.29&19.46\\\hline
\textbf{  5}&18.60&23.55&25.65&22.73&19.56\\\hline
\textbf{  6}&18.60&23.26&25.32&23.59&19.77\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&23.11&21.07&15.85&14.56\\\hline
\textbf{  3}&14.16&22.58&23.01&16.79&14.78\\\hline
\textbf{  4}&14.16&22.18&23.49&17.79&14.99\\\hline
\textbf{4.5}&14.16&22.02&23.47&18.31&15.10\\\hline
\textbf{  5}&14.16&21.88&23.39&18.84&15.21\\\hline
\textbf{  6}&14.16&21.65&23.16&19.91&15.44\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&20.26&16.03&9.94&8.57\\\hline
\textbf{  3}&8.13&19.94&18.99&10.97&8.80\\\hline
\textbf{  4}&8.14&19.57&20.21&12.09&9.03\\\hline
\textbf{4.5}&8.14&19.40&20.41&12.69&9.15\\\hline
\textbf{  5}&8.14&19.24&20.47&13.30&9.27\\\hline
\textbf{  6}&8.14&18.95&20.43&14.60&9.51\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/CURV_house.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{HOUSE with CURV}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&37.80&37.53&35.06&34.39\\\hline
\textbf{  3}&34.16&37.05&38.24&35.51&34.51\\\hline
\textbf{  4}&34.16&36.44&38.34&35.96&34.63\\\hline
\textbf{4.5}&34.16&36.18&38.27&36.18&34.69\\\hline
\textbf{  5}&34.16&35.95&38.17&36.40&34.75\\\hline
\textbf{  6}&34.16&35.55&37.91&36.80&34.87\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.14&34.09&32.83&29.32&28.46\\\hline
\textbf{  3}&28.15&33.49&34.06&29.94&28.62\\\hline
\textbf{  4}&28.15&32.99&34.40&30.58&28.78\\\hline
\textbf{4.5}&28.15&32.78&34.39&30.90&28.86\\\hline
\textbf{  5}&28.15&32.60&34.32&31.22&28.94\\\hline
\textbf{  6}&28.15&32.27&34.11&31.84&29.11\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.62&31.88&29.93&25.91&24.96\\\hline
\textbf{  3}&24.62&31.39&31.49&26.61&25.14\\\hline
\textbf{  4}&24.62&30.94&32.01&27.33&25.32\\\hline
\textbf{4.5}&24.62&30.75&32.05&27.70&25.41\\\hline
\textbf{  5}&24.63&30.57&32.02&28.08&25.51\\\hline
\textbf{  6}&24.63&30.26&31.85&28.82&25.69\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&30.24&27.79&23.47&22.48\\\hline
\textbf{  3}&22.12&29.81&29.59&24.21&22.67\\\hline
\textbf{  4}&22.12&29.39&30.25&24.99&22.86\\\hline
\textbf{4.5}&22.12&29.21&30.33&25.39&22.95\\\hline
\textbf{  5}&22.12&29.05&30.33&25.80&23.05\\\hline
\textbf{  6}&22.13&28.76&30.20&26.62&23.25\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.19&28.88&26.12&21.59&20.57\\\hline
\textbf{  3}&20.19&28.52&28.07&22.37&20.76\\\hline
\textbf{  4}&20.20&28.15&28.83&23.18&20.96\\\hline
\textbf{4.5}&20.20&27.99&28.94&23.60&21.06\\\hline
\textbf{  5}&20.20&27.86&28.95&24.04&21.17\\\hline
\textbf{  6}&20.21&27.62&28.85&24.91&21.37\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&27.75&24.66&20.01&18.97\\\hline
\textbf{  3}&18.59&27.45&26.76&20.80&19.17\\\hline
\textbf{  4}&18.59&27.14&27.63&21.64&19.37\\\hline
\textbf{4.5}&18.60&27.01&27.77&22.07&19.48\\\hline
\textbf{  5}&18.60&26.89&27.81&22.52&19.58\\\hline
\textbf{  6}&18.60&26.71&27.75&23.43&19.79\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&24.46&20.61&15.65&14.57\\\hline
\textbf{  3}&14.17&24.42&23.01&16.48&14.78\\\hline
\textbf{  4}&14.17&24.31&24.13&17.38&14.99\\\hline
\textbf{4.5}&14.17&24.26&24.36&17.84&15.10\\\hline
\textbf{  5}&14.18&24.23&24.48&18.33&15.21\\\hline
\textbf{  6}&14.18&24.19&24.53&19.33&15.43\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.14&19.51&14.85&9.66&8.55\\\hline
\textbf{  3}&8.14&19.74&17.53&10.52&8.77\\\hline
\textbf{  4}&8.15&19.76&18.93&11.45&8.99\\\hline
\textbf{4.5}&8.15&19.76&19.27&11.94&9.10\\\hline
\textbf{  5}&8.15&19.76&19.48&12.45&9.21\\\hline
\textbf{  6}&8.16&19.76&19.67&13.52&9.44\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/CURV_lena512x512.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{LENA512X512 with CURV}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&37.27&37.64&35.19&34.40\\\hline
\textbf{  3}&34.15&36.50&38.09&35.70&34.53\\\hline
\textbf{  4}&34.15&35.94&37.94&36.19&34.65\\\hline
\textbf{4.5}&34.15&35.71&37.79&36.43&34.72\\\hline
\textbf{  5}&34.15&35.51&37.63&36.65&34.78\\\hline
\textbf{  6}&34.15&35.15&37.31&37.06&34.91\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&34.29&33.52&29.56&28.47\\\hline
\textbf{  3}&28.13&33.56&34.65&30.31&28.65\\\hline
\textbf{  4}&28.13&32.99&34.78&31.08&28.83\\\hline
\textbf{4.5}&28.13&32.75&34.70&31.46&28.92\\\hline
\textbf{  5}&28.13&32.53&34.57&31.84&29.01\\\hline
\textbf{  6}&28.13&32.15&34.29&32.57&29.19\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.60&32.46&30.91&26.18&24.98\\\hline
\textbf{  3}&24.61&31.74&32.52&27.04&25.18\\\hline
\textbf{  4}&24.61&31.17&32.86&27.93&25.38\\\hline
\textbf{4.5}&24.61&30.93&32.81&28.39&25.48\\\hline
\textbf{  5}&24.61&30.72&32.70&28.85&25.58\\\hline
\textbf{  6}&24.61&30.35&32.43&29.76&25.78\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.12&31.13&28.98&23.78&22.51\\\hline
\textbf{  3}&22.12&30.45&30.94&24.70&22.72\\\hline
\textbf{  4}&22.12&29.90&31.44&25.67&22.93\\\hline
\textbf{4.5}&22.12&29.67&31.43&26.17&23.04\\\hline
\textbf{  5}&22.12&29.47&31.34&26.68&23.15\\\hline
\textbf{  6}&22.12&29.13&31.08&27.71&23.36\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.18&30.08&27.40&21.89&20.59\\\hline
\textbf{  3}&20.18&29.45&29.65&22.85&20.80\\\hline
\textbf{  4}&20.18&28.93&30.32&23.87&21.02\\\hline
\textbf{4.5}&20.18&28.71&30.34&24.40&21.13\\\hline
\textbf{  5}&20.18&28.52&30.27&24.95&21.24\\\hline
\textbf{  6}&20.19&28.20&30.03&26.06&21.47\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&29.21&26.07&20.34&19.01\\\hline
\textbf{  3}&18.59&28.63&28.56&21.32&19.23\\\hline
\textbf{  4}&18.60&28.14&29.37&22.37&19.45\\\hline
\textbf{4.5}&18.60&27.94&29.42&22.93&19.57\\\hline
\textbf{  5}&18.60&27.77&29.38&23.50&19.68\\\hline
\textbf{  6}&18.60&27.48&29.16&24.67&19.91\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&26.77&22.19&15.97&14.59\\\hline
\textbf{  3}&14.15&26.43&25.31&17.00&14.82\\\hline
\textbf{  4}&14.16&26.08&26.61&18.12&15.05\\\hline
\textbf{4.5}&14.16&25.94&26.80&18.72&15.17\\\hline
\textbf{  5}&14.16&25.82&26.85&19.35&15.29\\\hline
\textbf{  6}&14.16&25.63&26.74&20.66&15.53\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.14&23.15&16.65&10.01&8.59\\\hline
\textbf{  3}&8.14&23.28&20.45&11.09&8.82\\\hline
\textbf{  4}&8.14&23.18&22.47&12.27&9.07\\\hline
\textbf{4.5}&8.14&23.13&22.92&12.91&9.19\\\hline
\textbf{  5}&8.14&23.10&23.15&13.58&9.31\\\hline
\textbf{  6}&8.15&23.04&23.29&15.01&9.57\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/CURV_peppers256.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{PEPPERS256 with CURV}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&36.58&36.62&34.81&34.31\\\hline
\textbf{  3}&34.15&35.79&37.08&35.13&34.39\\\hline
\textbf{  4}&34.15&35.16&37.08&35.43&34.47\\\hline
\textbf{4.5}&34.15&34.90&36.99&35.58&34.51\\\hline
\textbf{  5}&34.15&34.66&36.86&35.72&34.55\\\hline
\textbf{  6}&34.15&34.25&36.57&35.98&34.62\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&32.86&32.05&29.13&28.38\\\hline
\textbf{  3}&28.13&32.18&32.96&29.64&28.51\\\hline
\textbf{  4}&28.13&31.63&33.14&30.15&28.64\\\hline
\textbf{4.5}&28.13&31.39&33.09&30.40&28.71\\\hline
\textbf{  5}&28.14&31.18&33.00&30.65&28.77\\\hline
\textbf{  6}&28.14&30.82&32.75&31.12&28.90\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.62&30.70&29.31&25.78&24.92\\\hline
\textbf{  3}&24.62&30.10&30.54&26.39&25.08\\\hline
\textbf{  4}&24.63&29.59&30.86&27.01&25.23\\\hline
\textbf{4.5}&24.63&29.38&30.84&27.33&25.31\\\hline
\textbf{  5}&24.63&29.19&30.77&27.64&25.39\\\hline
\textbf{  6}&24.63&28.85&30.55&28.24&25.54\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.12&29.12&27.26&23.37&22.44\\\hline
\textbf{  3}&22.12&28.59&28.71&24.03&22.61\\\hline
\textbf{  4}&22.12&28.12&29.17&24.72&22.78\\\hline
\textbf{4.5}&22.12&27.92&29.19&25.07&22.87\\\hline
\textbf{  5}&22.13&27.73&29.15&25.42&22.95\\\hline
\textbf{  6}&22.13&27.41&28.97&26.12&23.13\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&27.85&25.61&21.47&20.51\\\hline
\textbf{  3}&20.17&27.38&27.25&22.17&20.69\\\hline
\textbf{  4}&20.17&26.93&27.82&22.91&20.87\\\hline
\textbf{4.5}&20.17&26.74&27.87&23.29&20.96\\\hline
\textbf{  5}&20.18&26.56&27.85&23.66&21.05\\\hline
\textbf{  6}&20.18&26.25&27.70&24.42&21.23\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.60&26.77&24.27&19.95&18.96\\\hline
\textbf{  3}&18.60&26.33&26.05&20.68&19.14\\\hline
\textbf{  4}&18.60&25.90&26.69&21.45&19.33\\\hline
\textbf{4.5}&18.61&25.72&26.77&21.85&19.42\\\hline
\textbf{  5}&18.61&25.54&26.76&22.25&19.52\\\hline
\textbf{  6}&18.61&25.24&26.62&23.06&19.71\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&23.57&20.33&15.60&14.55\\\hline
\textbf{  3}&14.17&23.27&22.47&16.39&14.75\\\hline
\textbf{  4}&14.17&22.94&23.36&17.24&14.95\\\hline
\textbf{4.5}&14.17&22.80&23.51&17.68&15.05\\\hline
\textbf{  5}&14.17&22.68&23.55&18.13&15.16\\\hline
\textbf{  6}&14.18&22.49&23.47&19.05&15.37\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.14&18.91&14.70&9.64&8.54\\\hline
\textbf{  3}&8.14&18.99&17.23&10.48&8.76\\\hline
\textbf{  4}&8.15&18.95&18.45&11.39&8.97\\\hline
\textbf{4.5}&8.15&18.94&18.72&11.87&9.08\\\hline
\textbf{  5}&8.15&18.93&18.87&12.36&9.19\\\hline
\textbf{  6}&8.16&18.91&18.97&13.39&9.41\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/DWT_barbara512x512.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{BARBARA512X512 with DWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&34.02&36.73&35.40&34.44\\\hline
\textbf{  3}&34.15&32.87&36.14&35.93&34.58\\\hline
\textbf{  4}&34.15&32.01&35.51&36.35&34.72\\\hline
\textbf{4.5}&34.15&31.65&35.23&36.50&34.78\\\hline
\textbf{  5}&34.15&31.32&34.96&36.61&34.85\\\hline
\textbf{  6}&34.15&30.74&34.48&36.70&34.99\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&30.47&32.41&29.53&28.45\\\hline
\textbf{  3}&28.13&29.32&32.33&30.22&28.61\\\hline
\textbf{  4}&28.13&28.47&31.84&30.87&28.77\\\hline
\textbf{4.5}&28.13&28.12&31.58&31.17&28.85\\\hline
\textbf{  5}&28.13&27.81&31.33&31.45&28.94\\\hline
\textbf{  6}&28.13&27.28&30.87&31.90&29.10\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&28.27&29.74&26.08&24.95\\\hline
\textbf{  3}&24.61&27.18&30.04&26.85&25.12\\\hline
\textbf{  4}&24.61&26.37&29.63&27.62&25.30\\\hline
\textbf{4.5}&24.61&26.04&29.37&27.99&25.38\\\hline
\textbf{  5}&24.61&25.75&29.12&28.34&25.47\\\hline
\textbf{  6}&24.61&25.25&28.64&28.98&25.65\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&26.80&27.79&23.63&22.46\\\hline
\textbf{  3}&22.11&25.75&28.43&24.44&22.64\\\hline
\textbf{  4}&22.11&24.98&28.10&25.28&22.82\\\hline
\textbf{4.5}&22.11&24.68&27.85&25.69&22.91\\\hline
\textbf{  5}&22.11&24.41&27.60&26.10&23.01\\\hline
\textbf{  6}&22.11&23.95&27.13&26.87&23.19\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&25.68&26.26&21.73&20.54\\\hline
\textbf{  3}&20.17&24.68&27.20&22.58&20.72\\\hline
\textbf{  4}&20.18&23.98&26.95&23.46&20.91\\\hline
\textbf{4.5}&20.18&23.70&26.72&23.91&21.01\\\hline
\textbf{  5}&20.18&23.45&26.47&24.36&21.10\\\hline
\textbf{  6}&20.18&23.06&26.01&25.23&21.30\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&24.80&25.05&20.19&18.96\\\hline
\textbf{  3}&18.59&23.85&26.22&21.08&19.15\\\hline
\textbf{  4}&18.59&23.20&26.04&22.01&19.35\\\hline
\textbf{4.5}&18.59&22.96&25.80&22.48&19.45\\\hline
\textbf{  5}&18.59&22.75&25.56&22.96&19.55\\\hline
\textbf{  6}&18.60&22.42&25.10&23.92&19.75\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&22.73&21.54&15.84&14.54\\\hline
\textbf{  3}&14.15&22.07&23.58&16.80&14.75\\\hline
\textbf{  4}&14.16&21.65&23.71&17.84&14.96\\\hline
\textbf{4.5}&14.16&21.50&23.53&18.39&15.06\\\hline
\textbf{  5}&14.16&21.37&23.32&18.95&15.17\\\hline
\textbf{  6}&14.16&21.15&22.92&20.12&15.39\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&20.75&16.66&9.93&8.55\\\hline
\textbf{  3}&8.14&20.37&20.25&10.97&8.76\\\hline
\textbf{  4}&8.14&20.01&21.22&12.13&8.99\\\hline
\textbf{4.5}&8.14&19.87&21.22&12.76&9.10\\\hline
\textbf{  5}&8.14&19.73&21.12&13.43&9.21\\\hline
\textbf{  6}&8.14&19.50&20.90&14.86&9.45\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/DWT_boat.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{BOAT with DWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&33.54&36.24&35.33&34.44\\\hline
\textbf{  3}&34.15&32.58&35.42&35.81&34.58\\\hline
\textbf{  4}&34.15&31.87&34.73&36.18&34.71\\\hline
\textbf{4.5}&34.15&31.58&34.46&36.31&34.78\\\hline
\textbf{  5}&34.15&31.31&34.22&36.39&34.85\\\hline
\textbf{  6}&34.15&30.85&33.80&36.43&34.98\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&30.95&32.39&29.46&28.44\\\hline
\textbf{  3}&28.13&30.01&32.43&30.13&28.60\\\hline
\textbf{  4}&28.13&29.31&32.00&30.78&28.76\\\hline
\textbf{4.5}&28.13&29.03&31.77&31.08&28.84\\\hline
\textbf{  5}&28.13&28.77&31.55&31.37&28.92\\\hline
\textbf{  6}&28.13&28.33&31.15&31.86&29.08\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&29.14&29.88&26.06&24.95\\\hline
\textbf{  3}&24.61&28.22&30.42&26.83&25.12\\\hline
\textbf{  4}&24.61&27.55&30.11&27.60&25.30\\\hline
\textbf{4.5}&24.61&27.27&29.89&27.99&25.39\\\hline
\textbf{  5}&24.61&27.03&29.67&28.36&25.47\\\hline
\textbf{  6}&24.61&26.61&29.25&29.06&25.65\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&27.87&28.01&23.62&22.46\\\hline
\textbf{  3}&22.11&26.99&28.97&24.44&22.65\\\hline
\textbf{  4}&22.11&26.36&28.78&25.29&22.83\\\hline
\textbf{4.5}&22.11&26.10&28.57&25.72&22.92\\\hline
\textbf{  5}&22.11&25.87&28.36&26.15&23.02\\\hline
\textbf{  6}&22.12&25.49&27.94&26.99&23.21\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.18&26.90&26.58&21.76&20.55\\\hline
\textbf{  3}&20.18&26.07&27.85&22.62&20.74\\\hline
\textbf{  4}&20.18&25.47&27.76&23.53&20.93\\\hline
\textbf{4.5}&20.18&25.22&27.56&24.00&21.03\\\hline
\textbf{  5}&20.18&25.01&27.35&24.48&21.13\\\hline
\textbf{  6}&20.18&24.65&26.94&25.42&21.32\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.60&26.13&25.36&20.21&18.97\\\hline
\textbf{  3}&18.60&25.35&26.93&21.11&19.17\\\hline
\textbf{  4}&18.60&24.77&26.93&22.07&19.37\\\hline
\textbf{4.5}&18.60&24.54&26.75&22.56&19.47\\\hline
\textbf{  5}&18.60&24.34&26.55&23.07&19.57\\\hline
\textbf{  6}&18.60&23.99&26.16&24.10&19.77\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&24.14&21.89&15.87&14.55\\\hline
\textbf{  3}&14.16&23.48&24.42&16.85&14.76\\\hline
\textbf{  4}&14.16&22.98&24.83&17.92&14.97\\\hline
\textbf{4.5}&14.16&22.79&24.71&18.49&15.08\\\hline
\textbf{  5}&14.16&22.62&24.55&19.09&15.19\\\hline
\textbf{  6}&14.16&22.34&24.20&20.34&15.41\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.14&21.85&16.81&9.93&8.55\\\hline
\textbf{  3}&8.14&21.47&20.91&10.98&8.77\\\hline
\textbf{  4}&8.14&21.10&22.31&12.14&8.99\\\hline
\textbf{4.5}&8.14&20.96&22.36&12.78&9.10\\\hline
\textbf{  5}&8.14&20.83&22.28&13.45&9.22\\\hline
\textbf{  6}&8.14&20.61&22.04&14.92&9.45\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/DWT_fingerprint.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{FINGERPRINT with DWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&33.09&35.79&34.88&34.34\\\hline
\textbf{  3}&34.15&31.97&35.36&35.19&34.43\\\hline
\textbf{  4}&34.15&31.19&34.69&35.46&34.52\\\hline
\textbf{4.5}&34.15&30.87&34.35&35.57&34.57\\\hline
\textbf{  5}&34.15&30.59&34.03&35.67&34.61\\\hline
\textbf{  6}&34.15&30.10&33.46&35.81&34.70\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&29.62&31.26&29.17&28.39\\\hline
\textbf{  3}&28.14&28.64&31.29&29.68&28.52\\\hline
\textbf{  4}&28.14&27.90&30.88&30.16&28.65\\\hline
\textbf{4.5}&28.14&27.59&30.66&30.39&28.72\\\hline
\textbf{  5}&28.14&27.31&30.45&30.60&28.78\\\hline
\textbf{  6}&28.14&26.82&30.07&30.97&28.91\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&27.53&28.70&25.83&24.91\\\hline
\textbf{  3}&24.62&26.56&29.09&26.46&25.06\\\hline
\textbf{  4}&24.62&25.84&28.82&27.07&25.21\\\hline
\textbf{4.5}&24.62&25.55&28.63&27.37&25.29\\\hline
\textbf{  5}&24.62&25.28&28.43&27.67&25.37\\\hline
\textbf{  6}&24.62&24.83&28.05&28.21&25.52\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&26.05&26.88&23.44&22.43\\\hline
\textbf{  3}&22.11&25.12&27.53&24.14&22.59\\\hline
\textbf{  4}&22.11&24.43&27.34&24.86&22.76\\\hline
\textbf{4.5}&22.11&24.15&27.14&25.21&22.84\\\hline
\textbf{  5}&22.11&23.90&26.94&25.56&22.93\\\hline
\textbf{  6}&22.11&23.47&26.53&26.23&23.10\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&24.92&25.48&21.60&20.51\\\hline
\textbf{  3}&20.17&24.03&26.34&22.36&20.68\\\hline
\textbf{  4}&20.17&23.36&26.18&23.15&20.86\\\hline
\textbf{4.5}&20.17&23.09&25.99&23.54&20.95\\\hline
\textbf{  5}&20.17&22.84&25.78&23.94&21.04\\\hline
\textbf{  6}&20.17&22.42&25.37&24.71&21.22\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.60&24.05&24.31&20.08&18.95\\\hline
\textbf{  3}&18.60&23.17&25.37&20.89&19.13\\\hline
\textbf{  4}&18.60&22.52&25.26&21.72&19.32\\\hline
\textbf{4.5}&18.60&22.25&25.07&22.15&19.41\\\hline
\textbf{  5}&18.60&22.00&24.87&22.58&19.50\\\hline
\textbf{  6}&18.60&21.58&24.48&23.43&19.69\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&21.66&20.92&15.77&14.53\\\hline
\textbf{  3}&14.16&20.81&22.69&16.67&14.73\\\hline
\textbf{  4}&14.16&20.16&22.83&17.64&14.93\\\hline
\textbf{4.5}&14.16&19.88&22.69&18.14&15.03\\\hline
\textbf{  5}&14.16&19.64&22.51&18.66&15.13\\\hline
\textbf{  6}&14.16&19.22&22.16&19.73&15.34\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&18.56&16.14&9.88&8.54\\\hline
\textbf{  3}&8.14&17.78&19.08&10.88&8.75\\\hline
\textbf{  4}&8.14&17.19&19.71&11.99&8.97\\\hline
\textbf{4.5}&8.14&16.96&19.61&12.58&9.08\\\hline
\textbf{  5}&8.14&16.77&19.44&13.21&9.19\\\hline
\textbf{  6}&8.14&16.45&19.06&14.54&9.41\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/DWT_house.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{HOUSE with DWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&36.00&37.39&35.08&34.36\\\hline
\textbf{  3}&34.16&35.04&37.61&35.53&34.46\\\hline
\textbf{  4}&34.16&34.38&37.29&35.95&34.56\\\hline
\textbf{4.5}&34.16&34.11&37.07&36.16&34.61\\\hline
\textbf{  5}&34.16&33.88&36.84&36.35&34.66\\\hline
\textbf{  6}&34.16&33.47&36.38&36.69&34.77\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.14&32.73&32.65&29.28&28.40\\\hline
\textbf{  3}&28.14&31.92&33.50&29.87&28.53\\\hline
\textbf{  4}&28.14&31.27&33.44&30.46&28.66\\\hline
\textbf{4.5}&28.15&30.99&33.28&30.76&28.73\\\hline
\textbf{  5}&28.15&30.73&33.10&31.05&28.79\\\hline
\textbf{  6}&28.15&30.29&32.73&31.60&28.93\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&30.79&29.84&25.87&24.90\\\hline
\textbf{  3}&24.62&29.98&31.17&26.53&25.05\\\hline
\textbf{  4}&24.62&29.31&31.32&27.22&25.20\\\hline
\textbf{4.5}&24.62&29.03&31.20&27.57&25.27\\\hline
\textbf{  5}&24.62&28.77&31.04&27.92&25.35\\\hline
\textbf{  6}&24.63&28.33&30.69&28.62&25.50\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.10&29.40&27.79&23.42&22.40\\\hline
\textbf{  3}&22.10&28.59&29.51&24.14&22.56\\\hline
\textbf{  4}&22.11&27.94&29.85&24.89&22.72\\\hline
\textbf{4.5}&22.11&27.67&29.76&25.28&22.80\\\hline
\textbf{  5}&22.11&27.43&29.62&25.67&22.88\\\hline
\textbf{  6}&22.11&27.02&29.27&26.46&23.04\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.18&28.31&26.24&21.56&20.49\\\hline
\textbf{  3}&20.18&27.53&28.25&22.32&20.66\\\hline
\textbf{  4}&20.18&26.90&28.73&23.12&20.83\\\hline
\textbf{4.5}&20.19&26.64&28.66&23.54&20.91\\\hline
\textbf{  5}&20.19&26.40&28.52&23.96&21.00\\\hline
\textbf{  6}&20.19&25.99&28.17&24.83&21.17\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.61&27.48&24.96&20.03&18.94\\\hline
\textbf{  3}&18.62&26.74&27.26&20.82&19.11\\\hline
\textbf{  4}&18.62&26.11&27.90&21.66&19.28\\\hline
\textbf{4.5}&18.62&25.85&27.86&22.10&19.37\\\hline
\textbf{  5}&18.62&25.62&27.73&22.55&19.46\\\hline
\textbf{  6}&18.63&25.20&27.39&23.48&19.64\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&25.07&21.15&15.67&14.50\\\hline
\textbf{  3}&14.16&24.44&24.21&16.52&14.69\\\hline
\textbf{  4}&14.17&23.84&25.35&17.44&14.87\\\hline
\textbf{4.5}&14.17&23.60&25.41&17.93&14.97\\\hline
\textbf{  5}&14.17&23.38&25.32&18.44&15.06\\\hline
\textbf{  6}&14.18&23.03&25.02&19.52&15.26\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.16&22.06&15.67&9.71&8.51\\\hline
\textbf{  3}&8.17&21.78&19.80&10.60&8.70\\\hline
\textbf{  4}&8.17&21.28&22.10&11.58&8.90\\\hline
\textbf{4.5}&8.17&21.06&22.48&12.11&8.99\\\hline
\textbf{  5}&8.18&20.86&22.57&12.66&9.09\\\hline
\textbf{  6}&8.18&20.52&22.42&13.86&9.29\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/DWT_lena512x512.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{LENA512X512 with DWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.16&35.71&37.63&35.44&34.46\\\hline
\textbf{  3}&34.16&34.86&37.30&36.06&34.61\\\hline
\textbf{  4}&34.16&34.23&36.77&36.61&34.76\\\hline
\textbf{4.5}&34.16&33.97&36.54&36.86&34.83\\\hline
\textbf{  5}&34.16&33.74&36.32&37.08&34.91\\\hline
\textbf{  6}&34.16&33.32&35.94&37.42&35.06\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&32.93&33.48&29.59&28.47\\\hline
\textbf{  3}&28.13&32.09&34.07&30.36&28.64\\\hline
\textbf{  4}&28.13&31.45&33.81&31.14&28.81\\\hline
\textbf{4.5}&28.13&31.18&33.61&31.52&28.90\\\hline
\textbf{  5}&28.13&30.94&33.42&31.90&28.99\\\hline
\textbf{  6}&28.13&30.52&33.05&32.61&29.17\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&31.14&30.85&26.17&24.97\\\hline
\textbf{  3}&24.62&30.31&32.03&27.01&25.16\\\hline
\textbf{  4}&24.62&29.66&31.95&27.90&25.35\\\hline
\textbf{4.5}&24.62&29.39&31.78&28.36&25.44\\\hline
\textbf{  5}&24.62&29.15&31.59&28.81&25.54\\\hline
\textbf{  6}&24.62&28.72&31.23&29.71&25.73\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&29.83&28.89&23.72&22.48\\\hline
\textbf{  3}&22.11&29.00&30.52&24.61&22.67\\\hline
\textbf{  4}&22.11&28.35&30.60&25.56&22.87\\\hline
\textbf{4.5}&22.11&28.08&30.45&26.06&22.97\\\hline
\textbf{  5}&22.11&27.84&30.26&26.56&23.07\\\hline
\textbf{  6}&22.11&27.42&29.90&27.58&23.27\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&28.78&27.37&21.82&20.55\\\hline
\textbf{  3}&20.17&27.97&29.35&22.75&20.75\\\hline
\textbf{  4}&20.17&27.34&29.54&23.76&20.95\\\hline
\textbf{4.5}&20.17&27.08&29.40&24.28&21.06\\\hline
\textbf{  5}&20.17&26.85&29.22&24.82&21.16\\\hline
\textbf{  6}&20.17&26.45&28.86&25.93&21.37\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&27.98&26.12&20.28&18.98\\\hline
\textbf{  3}&18.59&27.18&28.40&21.24&19.18\\\hline
\textbf{  4}&18.59&26.55&28.71&22.28&19.39\\\hline
\textbf{4.5}&18.59&26.29&28.58&22.83&19.50\\\hline
\textbf{  5}&18.59&26.06&28.40&23.40&19.60\\\hline
\textbf{  6}&18.59&25.68&28.03&24.59&19.82\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&25.73&22.37&15.91&14.56\\\hline
\textbf{  3}&14.16&25.04&25.59&16.92&14.77\\\hline
\textbf{  4}&14.16&24.49&26.37&18.04&14.99\\\hline
\textbf{4.5}&14.16&24.27&26.30&18.64&15.10\\\hline
\textbf{  5}&14.16&24.07&26.15&19.27&15.21\\\hline
\textbf{  6}&14.16&23.75&25.80&20.62&15.43\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.15&23.01&17.09&9.96&8.56\\\hline
\textbf{  3}&8.15&22.55&21.64&11.03&8.78\\\hline
\textbf{  4}&8.15&22.06&23.42&12.22&9.01\\\hline
\textbf{4.5}&8.15&21.85&23.53&12.87&9.12\\\hline
\textbf{  5}&8.15&21.66&23.46&13.56&9.24\\\hline
\textbf{  6}&8.15&21.35&23.20&15.08&9.47\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/DWT_peppers256.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{PEPPERS256 with DWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.14&35.01&36.79&35.02&34.32\\\hline
\textbf{  3}&34.14&34.03&36.52&35.42&34.40\\\hline
\textbf{  4}&34.14&33.29&36.03&35.77&34.49\\\hline
\textbf{4.5}&34.14&32.98&35.79&35.92&34.53\\\hline
\textbf{  5}&34.14&32.69&35.56&36.06&34.57\\\hline
\textbf{  6}&34.14&32.20&35.15&36.27&34.66\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&31.65&32.17&29.21&28.36\\\hline
\textbf{  3}&28.13&30.71&32.62&29.74&28.48\\\hline
\textbf{  4}&28.13&29.98&32.40&30.27&28.59\\\hline
\textbf{4.5}&28.13&29.68&32.22&30.52&28.65\\\hline
\textbf{  5}&28.14&29.41&32.02&30.77&28.71\\\hline
\textbf{  6}&28.14&28.93&31.64&31.21&28.83\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.63&29.52&29.38&25.82&24.89\\\hline
\textbf{  3}&24.63&28.61&30.25&26.44&25.03\\\hline
\textbf{  4}&24.63&27.90&30.17&27.07&25.16\\\hline
\textbf{4.5}&24.63&27.60&30.01&27.38&25.23\\\hline
\textbf{  5}&24.64&27.33&29.83&27.68&25.30\\\hline
\textbf{  6}&24.64&26.87&29.45&28.27&25.44\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.13&28.07&27.31&23.38&22.41\\\hline
\textbf{  3}&22.13&27.20&28.54&24.04&22.55\\\hline
\textbf{  4}&22.13&26.49&28.64&24.72&22.70\\\hline
\textbf{4.5}&22.13&26.20&28.51&25.07&22.77\\\hline
\textbf{  5}&22.13&25.93&28.34&25.41&22.84\\\hline
\textbf{  6}&22.14&25.46&27.96&26.09&22.99\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&26.91&25.73&21.48&20.46\\\hline
\textbf{  3}&20.17&26.03&27.22&22.19&20.62\\\hline
\textbf{  4}&20.17&25.32&27.42&22.92&20.77\\\hline
\textbf{4.5}&20.18&25.02&27.30&23.30&20.85\\\hline
\textbf{  5}&20.18&24.75&27.13&23.67&20.93\\\hline
\textbf{  6}&20.18&24.26&26.76&24.43&21.09\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.60&25.94&24.42&19.95&18.91\\\hline
\textbf{  3}&18.61&25.08&26.14&20.69&19.07\\\hline
\textbf{  4}&18.61&24.37&26.44&21.46&19.23\\\hline
\textbf{4.5}&18.61&24.07&26.34&21.85&19.31\\\hline
\textbf{  5}&18.61&23.79&26.17&22.25&19.39\\\hline
\textbf{  6}&18.62&23.30&25.81&23.06&19.56\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&23.25&20.71&15.62&14.49\\\hline
\textbf{  3}&14.16&22.40&23.11&16.43&14.67\\\hline
\textbf{  4}&14.17&21.70&23.75&17.31&14.84\\\hline
\textbf{4.5}&14.17&21.41&23.69&17.76&14.94\\\hline
\textbf{  5}&14.17&21.17&23.55&18.24&15.03\\\hline
\textbf{  6}&14.17&20.77&23.16&19.22&15.21\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.14&20.05&15.45&9.68&8.49\\\hline
\textbf{  3}&8.15&19.56&18.98&10.57&8.68\\\hline
\textbf{  4}&8.15&19.10&20.44&11.53&8.87\\\hline
\textbf{4.5}&8.16&18.90&20.54&12.05&8.97\\\hline
\textbf{  5}&8.16&18.73&20.48&12.59&9.07\\\hline
\textbf{  6}&8.16&18.42&20.21&13.74&9.27\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/UDWT_barbara512x512.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{BARBARA512X512 with UDWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.16&36.64&36.90&35.00&34.36\\\hline
\textbf{  3}&34.16&35.85&37.35&35.41&34.45\\\hline
\textbf{  4}&34.16&35.13&37.38&35.81&34.55\\\hline
\textbf{4.5}&34.16&34.81&37.32&36.00&34.60\\\hline
\textbf{  5}&34.16&34.52&37.22&36.18&34.65\\\hline
\textbf{  6}&34.16&33.97&36.99&36.51&34.75\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&32.31&32.22&29.30&28.41\\\hline
\textbf{  3}&28.13&31.38&33.06&29.91&28.55\\\hline
\textbf{  4}&28.13&30.55&33.24&30.51&28.69\\\hline
\textbf{4.5}&28.13&30.19&33.20&30.81&28.76\\\hline
\textbf{  5}&28.13&29.85&33.11&31.10&28.83\\\hline
\textbf{  6}&28.13&29.26&32.85&31.65&28.97\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&29.74&29.44&25.95&24.92\\\hline
\textbf{  3}&24.61&28.76&30.54&26.65&25.08\\\hline
\textbf{  4}&24.61&27.90&30.81&27.37&25.25\\\hline
\textbf{4.5}&24.61&27.54&30.77&27.74&25.33\\\hline
\textbf{  5}&24.61&27.21&30.67&28.09&25.41\\\hline
\textbf{  6}&24.61&26.64&30.37&28.79&25.58\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&27.95&27.43&23.54&22.45\\\hline
\textbf{  3}&22.11&26.96&28.74&24.32&22.62\\\hline
\textbf{  4}&22.11&26.13&29.08&25.12&22.80\\\hline
\textbf{4.5}&22.11&25.79&29.04&25.52&22.89\\\hline
\textbf{  5}&22.11&25.48&28.94&25.93&22.97\\\hline
\textbf{  6}&22.11&24.97&28.62&26.72&23.15\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&26.64&25.86&21.67&20.52\\\hline
\textbf{  3}&20.17&25.71&27.35&22.49&20.70\\\hline
\textbf{  4}&20.17&24.95&27.77&23.34&20.89\\\hline
\textbf{4.5}&20.17&24.64&27.74&23.78&20.98\\\hline
\textbf{  5}&20.17&24.38&27.64&24.22&21.07\\\hline
\textbf{  6}&20.17&23.95&27.32&25.10&21.26\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&25.62&24.56&20.14&18.96\\\hline
\textbf{  3}&18.59&24.78&26.20&21.00&19.14\\\hline
\textbf{  4}&18.59&24.11&26.70&21.90&19.33\\\hline
\textbf{4.5}&18.59&23.85&26.69&22.36&19.43\\\hline
\textbf{  5}&18.59&23.64&26.60&22.83&19.53\\\hline
\textbf{  6}&18.59&23.29&26.29&23.77&19.73\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&23.31&20.87&15.83&14.54\\\hline
\textbf{  3}&14.15&22.90&23.04&16.76&14.75\\\hline
\textbf{  4}&14.15&22.52&23.90&17.77&14.95\\\hline
\textbf{4.5}&14.15&22.36&24.00&18.30&15.06\\\hline
\textbf{  5}&14.15&22.23&23.99&18.84&15.17\\\hline
\textbf{  6}&14.15&22.01&23.79&19.95&15.38\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&20.89&15.64&9.91&8.54\\\hline
\textbf{  3}&8.13&21.14&18.70&10.92&8.76\\\hline
\textbf{  4}&8.13&20.93&20.52&12.03&8.98\\\hline
\textbf{4.5}&8.13&20.81&21.00&12.63&9.09\\\hline
\textbf{  5}&8.13&20.69&21.29&13.24&9.21\\\hline
\textbf{  6}&8.13&20.48&21.51&14.53&9.44\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/UDWT_boat.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{BOAT with UDWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.16&35.96&36.61&34.93&34.34\\\hline
\textbf{  3}&34.16&35.14&36.90&35.30&34.43\\\hline
\textbf{  4}&34.16&34.49&36.76&35.65&34.52\\\hline
\textbf{4.5}&34.16&34.22&36.62&35.81&34.57\\\hline
\textbf{  5}&34.16&33.97&36.46&35.97&34.61\\\hline
\textbf{  6}&34.16&33.54&36.12&36.26&34.70\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&32.49&32.27&29.31&28.41\\\hline
\textbf{  3}&28.13&31.72&33.05&29.92&28.55\\\hline
\textbf{  4}&28.13&31.07&33.15&30.53&28.69\\\hline
\textbf{4.5}&28.13&30.80&33.08&30.83&28.77\\\hline
\textbf{  5}&28.13&30.55&32.97&31.13&28.84\\\hline
\textbf{  6}&28.13&30.11&32.70&31.68&28.98\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&30.50&29.68&25.99&24.93\\\hline
\textbf{  3}&24.61&29.77&30.84&26.72&25.10\\\hline
\textbf{  4}&24.61&29.14&31.12&27.48&25.27\\\hline
\textbf{4.5}&24.61&28.86&31.09&27.86&25.35\\\hline
\textbf{  5}&24.61&28.62&31.00&28.23&25.44\\\hline
\textbf{  6}&24.61&28.20&30.74&28.96&25.61\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&29.10&27.76&23.60&22.46\\\hline
\textbf{  3}&22.11&28.42&29.22&24.40&22.64\\\hline
\textbf{  4}&22.11&27.81&29.65&25.25&22.82\\\hline
\textbf{4.5}&22.11&27.55&29.66&25.68&22.91\\\hline
\textbf{  5}&22.11&27.32&29.59&26.11&23.01\\\hline
\textbf{  6}&22.11&26.92&29.36&26.96&23.19\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&28.04&26.24&21.73&20.54\\\hline
\textbf{  3}&20.17&27.44&27.94&22.59&20.73\\\hline
\textbf{  4}&20.17&26.86&28.52&23.50&20.92\\\hline
\textbf{4.5}&20.17&26.61&28.57&23.96&21.02\\\hline
\textbf{  5}&20.17&26.39&28.53&24.43&21.11\\\hline
\textbf{  6}&20.17&26.01&28.33&25.38&21.31\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&27.23&24.98&20.21&18.97\\\hline
\textbf{  3}&18.59&26.68&26.90&21.10&19.17\\\hline
\textbf{  4}&18.59&26.12&27.63&22.06&19.37\\\hline
\textbf{4.5}&18.59&25.88&27.72&22.55&19.47\\\hline
\textbf{  5}&18.59&25.67&27.71&23.05&19.57\\\hline
\textbf{  6}&18.59&25.31&27.53&24.07&19.78\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&24.99&21.26&15.88&14.56\\\hline
\textbf{  3}&14.16&24.71&23.82&16.85&14.77\\\hline
\textbf{  4}&14.16&24.25&25.08&17.90&14.98\\\hline
\textbf{4.5}&14.16&24.05&25.34&18.46&15.09\\\hline
\textbf{  5}&14.16&23.86&25.46&19.04&15.20\\\hline
\textbf{  6}&14.16&23.55&25.43&20.22&15.42\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&22.03&15.85&9.93&8.55\\\hline
\textbf{  3}&8.13&22.44&19.22&10.97&8.77\\\hline
\textbf{  4}&8.13&22.19&21.43&12.10&8.99\\\hline
\textbf{4.5}&8.13&22.05&22.09&12.71&9.11\\\hline
\textbf{  5}&8.13&21.90&22.51&13.34&9.22\\\hline
\textbf{  6}&8.13&21.65&22.89&14.68&9.46\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/UDWT_fingerprint.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{FINGERPRINT with UDWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&35.18&35.97&34.72&34.30\\\hline
\textbf{  3}&34.15&34.24&36.23&34.99&34.37\\\hline
\textbf{  4}&34.15&33.47&36.15&35.24&34.44\\\hline
\textbf{4.5}&34.15&33.15&36.03&35.36&34.47\\\hline
\textbf{  5}&34.15&32.87&35.89&35.48&34.51\\\hline
\textbf{  6}&34.15&32.37&35.55&35.69&34.57\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.13&31.05&31.33&29.09&28.37\\\hline
\textbf{  3}&28.13&30.25&31.87&29.57&28.48\\\hline
\textbf{  4}&28.13&29.58&31.87&30.05&28.60\\\hline
\textbf{4.5}&28.13&29.30&31.77&30.27&28.66\\\hline
\textbf{  5}&28.13&29.04&31.64&30.50&28.72\\\hline
\textbf{  6}&28.13&28.60&31.34&30.91&28.85\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&28.87&28.71&25.80&24.90\\\hline
\textbf{  3}&24.61&28.12&29.50&26.41&25.05\\\hline
\textbf{  4}&24.61&27.49&29.61&27.02&25.19\\\hline
\textbf{4.5}&24.61&27.22&29.54&27.32&25.27\\\hline
\textbf{  5}&24.61&26.97&29.43&27.62&25.34\\\hline
\textbf{  6}&24.61&26.55&29.16&28.19&25.49\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&27.38&26.82&23.43&22.43\\\hline
\textbf{  3}&22.11&26.68&27.84&24.13&22.59\\\hline
\textbf{  4}&22.11&26.07&28.05&24.83&22.76\\\hline
\textbf{4.5}&22.12&25.80&28.00&25.19&22.84\\\hline
\textbf{  5}&22.12&25.57&27.91&25.54&22.92\\\hline
\textbf{  6}&22.12&25.15&27.66&26.22&23.09\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&26.27&25.32&21.57&20.50\\\hline
\textbf{  3}&20.17&25.61&26.54&22.32&20.68\\\hline
\textbf{  4}&20.17&25.01&26.86&23.10&20.85\\\hline
\textbf{4.5}&20.17&24.74&26.84&23.49&20.94\\\hline
\textbf{  5}&20.17&24.51&26.77&23.88&21.03\\\hline
\textbf{  6}&20.17&24.08&26.54&24.65&21.21\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.58&25.35&24.08&20.05&18.94\\\hline
\textbf{  3}&18.58&24.73&25.47&20.85&19.12\\\hline
\textbf{  4}&18.58&24.13&25.90&21.67&19.30\\\hline
\textbf{4.5}&18.58&23.86&25.91&22.10&19.39\\\hline
\textbf{  5}&18.58&23.62&25.85&22.52&19.48\\\hline
\textbf{  6}&18.59&23.19&25.65&23.36&19.67\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.16&22.84&20.53&15.78&14.54\\\hline
\textbf{  3}&14.16&22.26&22.48&16.67&14.74\\\hline
\textbf{  4}&14.16&21.61&23.25&17.63&14.94\\\hline
\textbf{4.5}&14.16&21.32&23.36&18.13&15.04\\\hline
\textbf{  5}&14.16&21.06&23.37&18.64&15.15\\\hline
\textbf{  6}&14.16&20.58&23.23&19.66&15.36\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&19.32&15.36&9.87&8.54\\\hline
\textbf{  3}&8.13&18.92&18.09&10.86&8.75\\\hline
\textbf{  4}&8.13&18.31&19.50&11.93&8.97\\\hline
\textbf{4.5}&8.13&18.04&19.81&12.50&9.08\\\hline
\textbf{  5}&8.13&17.80&19.95&13.09&9.19\\\hline
\textbf{  6}&8.13&17.41&19.92&14.32&9.41\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/UDWT_house.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{HOUSE with UDWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.17&37.38&37.33&35.07&34.38\\\hline
\textbf{  3}&34.17&36.62&37.99&35.52&34.48\\\hline
\textbf{  4}&34.17&36.00&38.11&35.97&34.59\\\hline
\textbf{4.5}&34.17&35.74&38.05&36.18&34.64\\\hline
\textbf{  5}&34.17&35.50&37.95&36.40&34.69\\\hline
\textbf{  6}&34.17&35.10&37.67&36.80&34.80\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.14&33.91&32.62&29.32&28.41\\\hline
\textbf{  3}&28.14&33.34&33.85&29.94&28.55\\\hline
\textbf{  4}&28.14&32.77&34.30&30.58&28.69\\\hline
\textbf{4.5}&28.14&32.52&34.35&30.90&28.76\\\hline
\textbf{  5}&28.14&32.29&34.32&31.22&28.84\\\hline
\textbf{  6}&28.14&31.88&34.17&31.85&28.98\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.63&31.86&29.80&25.94&24.93\\\hline
\textbf{  3}&24.63&31.38&31.42&26.65&25.09\\\hline
\textbf{  4}&24.63&30.81&32.15&27.38&25.25\\\hline
\textbf{4.5}&24.63&30.55&32.28&27.76&25.33\\\hline
\textbf{  5}&24.63&30.32&32.31&28.14&25.41\\\hline
\textbf{  6}&24.63&29.89&32.22&28.90&25.57\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.12&30.41&27.72&23.50&22.44\\\hline
\textbf{  3}&22.12&29.98&29.65&24.26&22.61\\\hline
\textbf{  4}&22.12&29.42&30.60&25.06&22.78\\\hline
\textbf{4.5}&22.12&29.17&30.80&25.47&22.86\\\hline
\textbf{  5}&22.12&28.94&30.88&25.89&22.95\\\hline
\textbf{  6}&22.12&28.53&30.84&26.74&23.12\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&29.25&26.03&21.60&20.51\\\hline
\textbf{  3}&20.17&28.91&28.19&22.39&20.68\\\hline
\textbf{  4}&20.17&28.39&29.34&23.22&20.86\\\hline
\textbf{4.5}&20.17&28.14&29.60&23.66&20.94\\\hline
\textbf{  5}&20.17&27.92&29.73&24.10&21.03\\\hline
\textbf{  6}&20.18&27.52&29.74&25.01&21.21\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&28.32&24.67&20.06&18.94\\\hline
\textbf{  3}&18.59&28.08&27.00&20.87&19.11\\\hline
\textbf{  4}&18.59&27.58&28.30&21.73&19.29\\\hline
\textbf{4.5}&18.60&27.34&28.62&22.19&19.38\\\hline
\textbf{  5}&18.60&27.12&28.79&22.65&19.48\\\hline
\textbf{  6}&18.60&26.74&28.85&23.61&19.66\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&25.68&20.66&15.68&14.51\\\hline
\textbf{  3}&14.15&25.79&23.46&16.54&14.70\\\hline
\textbf{  4}&14.15&25.40&25.26&17.47&14.89\\\hline
\textbf{4.5}&14.15&25.19&25.79&17.96&14.98\\\hline
\textbf{  5}&14.15&24.99&26.13&18.46&15.08\\\hline
\textbf{  6}&14.15&24.63&26.40&19.52&15.28\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.11&21.90&14.99&9.69&8.48\\\hline
\textbf{  3}&8.12&22.75&18.28&10.59&8.68\\\hline
\textbf{  4}&8.12&22.54&20.78&11.56&8.87\\\hline
\textbf{4.5}&8.12&22.35&21.67&12.08&8.97\\\hline
\textbf{  5}&8.12&22.16&22.33&12.62&9.07\\\hline
\textbf{  6}&8.12&21.79&23.08&13.76&9.28\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/UDWT_lena512x512.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{LENA512X512 with UDWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&37.35&37.51&35.17&34.39\\\hline
\textbf{  3}&34.15&36.66&38.02&35.68&34.52\\\hline
\textbf{  4}&34.15&36.10&38.01&36.18&34.64\\\hline
\textbf{4.5}&34.15&35.86&37.91&36.41&34.70\\\hline
\textbf{  5}&34.15&35.65&37.79&36.64&34.77\\\hline
\textbf{  6}&34.15&35.27&37.52&37.07&34.89\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.14&34.23&33.24&29.53&28.47\\\hline
\textbf{  3}&28.14&33.61&34.44&30.27&28.63\\\hline
\textbf{  4}&28.14&33.04&34.77&31.03&28.80\\\hline
\textbf{4.5}&28.14&32.79&34.76&31.41&28.89\\\hline
\textbf{  5}&28.14&32.56&34.70&31.79&28.98\\\hline
\textbf{  6}&28.14&32.16&34.50&32.53&29.15\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&32.32&30.53&26.14&24.97\\\hline
\textbf{  3}&24.61&31.75&32.19&26.98&25.15\\\hline
\textbf{  4}&24.61&31.18&32.78&27.87&25.34\\\hline
\textbf{4.5}&24.61&30.93&32.85&28.32&25.44\\\hline
\textbf{  5}&24.61&30.70&32.83&28.78&25.53\\\hline
\textbf{  6}&24.61&30.29&32.67&29.69&25.73\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&30.96&28.53&23.73&22.49\\\hline
\textbf{  3}&22.11&30.45&30.53&24.63&22.69\\\hline
\textbf{  4}&22.11&29.89&31.34&25.59&22.89\\\hline
\textbf{4.5}&22.12&29.64&31.47&26.08&22.99\\\hline
\textbf{  5}&22.12&29.41&31.49&26.59&23.09\\\hline
\textbf{  6}&22.12&29.01&31.36&27.61&23.30\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.17&29.86&26.88&21.83&20.56\\\hline
\textbf{  3}&20.17&29.43&29.14&22.76&20.76\\\hline
\textbf{  4}&20.17&28.89&30.15&23.76&20.96\\\hline
\textbf{4.5}&20.17&28.65&30.34&24.28&21.07\\\hline
\textbf{  5}&20.17&28.43&30.40&24.82&21.17\\\hline
\textbf{  6}&20.17&28.04&30.32&25.92&21.39\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.58&28.98&25.52&20.28&18.98\\\hline
\textbf{  3}&18.58&28.63&27.99&21.23&19.18\\\hline
\textbf{  4}&18.58&28.10&29.18&22.26&19.39\\\hline
\textbf{4.5}&18.58&27.87&29.42&22.80&19.50\\\hline
\textbf{  5}&18.58&27.65&29.52&23.36&19.61\\\hline
\textbf{  6}&18.58&27.27&29.48&24.51&19.83\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.15&26.53&21.59&15.91&14.56\\\hline
\textbf{  3}&14.15&26.48&24.61&16.92&14.78\\\hline
\textbf{  4}&14.15&26.04&26.35&18.02&14.99\\\hline
\textbf{4.5}&14.15&25.82&26.80&18.61&15.10\\\hline
\textbf{  5}&14.15&25.62&27.05&19.21&15.22\\\hline
\textbf{  6}&14.15&25.27&27.19&20.49&15.45\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.13&23.06&16.00&9.95&8.55\\\hline
\textbf{  3}&8.13&23.74&19.61&10.99&8.77\\\hline
\textbf{  4}&8.13&23.49&22.18&12.15&9.00\\\hline
\textbf{4.5}&8.13&23.31&23.02&12.77&9.11\\\hline
\textbf{  5}&8.13&23.14&23.59&13.42&9.23\\\hline
\textbf{  6}&8.13&22.82&24.17&14.79&9.47\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/UDWT_peppers256.tex <==
\begin{center}
\begin{scriptsize}
\begin{tabular}{cc}
\multicolumn{2}{c}{PEPPERS256 with UDWT}
\\
$\sigma=5$ & $\sigma=10$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&34.15&37.02&36.83&34.90&34.32\\\hline
\textbf{  3}&34.15&36.35&37.37&35.27&34.40\\\hline
\textbf{  4}&34.15&35.75&37.48&35.62&34.48\\\hline
\textbf{4.5}&34.15&35.49&37.43&35.79&34.52\\\hline
\textbf{  5}&34.15&35.24&37.36&35.96&34.56\\\hline
\textbf{  6}&34.15&34.81&37.15&36.27&34.64\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&28.12&33.23&32.14&29.18&28.36\\\hline
\textbf{  3}&28.12&32.60&33.20&29.73&28.48\\\hline
\textbf{  4}&28.12&31.98&33.58&30.28&28.61\\\hline
\textbf{4.5}&28.12&31.70&33.61&30.56&28.67\\\hline
\textbf{  5}&28.12&31.44&33.57&30.83&28.73\\\hline
\textbf{  6}&28.12&30.97&33.41&31.36&28.85\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=15$ & $\sigma=20$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&24.61&30.95&29.33&25.82&24.89\\\hline
\textbf{  3}&24.61&30.35&30.71&26.46&25.03\\\hline
\textbf{  4}&24.61&29.71&31.27&27.12&25.17\\\hline
\textbf{4.5}&24.61&29.43&31.35&27.45&25.25\\\hline
\textbf{  5}&24.61&29.16&31.35&27.78&25.32\\\hline
\textbf{  6}&24.61&28.69&31.21&28.44&25.46\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&22.11&29.34&27.27&23.41&22.41\\\hline
\textbf{  3}&22.12&28.77&28.91&24.10&22.57\\\hline
\textbf{  4}&22.12&28.13&29.63&24.83&22.72\\\hline
\textbf{4.5}&22.12&27.84&29.75&25.19&22.80\\\hline
\textbf{  5}&22.12&27.57&29.78&25.57&22.88\\\hline
\textbf{  6}&22.12&27.08&29.66&26.31&23.04\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=25$ & $\sigma=30$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&20.16&28.04&25.59&21.50&20.47\\\hline
\textbf{  3}&20.16&27.51&27.42&22.23&20.63\\\hline
\textbf{  4}&20.16&26.86&28.29&23.00&20.79\\\hline
\textbf{4.5}&20.16&26.57&28.46&23.39&20.87\\\hline
\textbf{  5}&20.16&26.30&28.52&23.79&20.96\\\hline
\textbf{  6}&20.16&25.80&28.44&24.59&21.12\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&18.59&27.03&24.25&19.97&18.91\\\hline
\textbf{  3}&18.59&26.53&26.25&20.73&19.07\\\hline
\textbf{  4}&18.59&25.88&27.25&21.53&19.24\\\hline
\textbf{4.5}&18.59&25.58&27.46&21.94&19.33\\\hline
\textbf{  5}&18.59&25.30&27.55&22.37&19.41\\\hline
\textbf{  6}&18.59&24.80&27.50&23.22&19.59\\\hline
\end{tabular}
\end{scriptsize}\\
$\sigma=50$ & $\sigma=100$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&14.17&24.10&20.37&15.65&14.51\\\hline
\textbf{  3}&14.17&23.74&22.80&16.47&14.69\\\hline
\textbf{  4}&14.17&23.14&24.17&17.35&14.87\\\hline
\textbf{4.5}&14.17&22.88&24.52&17.81&14.97\\\hline
\textbf{  5}&14.17&22.63&24.69&18.29&15.06\\\hline
\textbf{  6}&14.17&22.22&24.74&19.27&15.25\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
&\textbf{ 1}&\textbf{ 2}&\textbf{ 4}&\textbf{ 8}&\textbf{16}\\\hline
\textbf{  2}&8.14&20.45&14.85&9.70&8.51\\\hline
\textbf{  3}&8.14&20.74&17.83&10.58&8.70\\\hline
\textbf{  4}&8.14&20.43&19.86&11.53&8.89\\\hline
\textbf{4.5}&8.14&20.25&20.49&12.04&8.99\\\hline
\textbf{  5}&8.14&20.08&20.90&12.56&9.09\\\hline
\textbf{  6}&8.14&19.78&21.27&13.66&9.29\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}
\end{center}


==> images/compare_psnrbest.tex <==
\begin{scriptsize}
\begin{tabular}{c@{}@{}c}
Barbara $512 \times 512$ & Lena $512 \times 512$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|c|c|}
\hline
$\sigma$   & 5     & 10    & 15    & 20    & 25    & 30    & 50\\
\psnrin    & 34.15 & 28.13 & 24.61 & 22.11 & 20.17 & 18.59 & 14.15\\\hline\hline
\textbf{DWT}&36.73&32.41&30.04&28.43&27.20&26.22&23.71\\\hline
\textbf{UDWT}&37.38&33.24&30.81&29.08&27.77&26.70&24.00\\\hline
\textbf{CURV}&37.57&33.68&31.53&29.99&28.82&27.86&25.18\\\hline
\textbf{BLS}    &34.57&28.52&24.57&22.46&20.95&19.56&15.99\\\hline
%\textbf{Surelet}&36.59&32.04&29.51&27.82&26.61&25.68&23.53\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
5     & 10    & 15    & 20    & 25    & 30    & 50\\
34.15 & 28.13 & 24.61 & 22.11 & 20.17 & 18.59 & 14.15\\\hline\hline
37.63&34.07&32.03&30.60&29.54&28.71&26.37\\\hline
38.02&34.77&32.85&31.49&30.40&29.52&27.19\\\hline
38.09&34.78&32.86&31.44&30.34&29.42&26.85\\\hline
34.85&28.43&25.30&23.19&21.64&20.29&16.32\\\hline
%37.80&34.37&32.47&31.15&30.15&29.32&27.15\\\hline
\end{tabular}
\end{scriptsize}\\
House $256 \times 256$ & Boat $512 \times 512$\\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{DWT}&37.61&33.50&31.32&29.85&28.73&27.90&25.41\\\hline
\textbf{UDWT}&38.11&34.35&32.31&30.88&29.74&28.85&26.40\\\hline
\textbf{CURV}&38.34&34.40&32.05&30.33&28.95&27.81&24.53\\\hline
\textbf{BLS}&38.43&35.08&33.34&32.12&31.12&30.33&27.94\\\hline
%\textbf{Surelet}&37.71&34.11&32.16&30.78&29.77&28.88&26.52\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
36.43&32.43&30.42&28.97&27.85&26.93&24.83\\\hline
36.90&33.15&31.12&29.66&28.57&27.72&25.46\\\hline
36.88&33.09&31.03&29.65&28.58&27.70&25.32\\\hline
34.54&28.25&24.86&22.58&21.03&19.74&16.04\\\hline
%36.69&32.90&30.86&29.48&28.45&27.65&25.56\\\hline
\end{tabular}
\end{scriptsize}\\
Fingerprint $512 \times 512$ & Peppers $256 \times 256$ \\
\begin{scriptsize}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{DWT}&35.81&31.29&29.09&27.53&26.34&25.37&22.83\\\hline
\textbf{UDWT}&36.23&31.87&29.61&28.05&26.86&25.91&23.37\\\hline
\textbf{CURV}&36.13&31.98&29.65&28.04&26.84&25.92&23.49\\\hline
\textbf{BLS}&34.09&27.86&24.16&21.94&20.31&19.02&15.48\\\hline
%\textbf{Surelet}&35.91&31.63&29.40&27.89&26.75&25.82&23.34\\\hline
\end{tabular}
\end{scriptsize}&
\begin{scriptsize}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
36.79&32.62&30.25&28.64&27.42&26.44&23.75\\\hline
37.48&33.61&31.35&29.78&28.52&27.55&24.74\\\hline
37.08&33.14&30.86&29.19&27.87&26.77&23.57\\\hline
37.30&33.76&31.75&30.31&29.23&28.33&25.94\\\hline
%37.21&33.22&30.87&29.40&28.16&27.22&24.48\\\hline
\end{tabular}
\end{scriptsize}\end{tabular}
\end{scriptsize}









